OpenRL: A Unified Reinforcement Learning Framework

We present OpenRL, an advanced reinforcement learning (RL) framework designed to accommodate a diverse array of tasks, from single-agent challenges to complex multi-agent systems. OpenRL's robust support for self-play training empowers agents to develop advanced strategies in competitive settings. Notably, OpenRL integrates Natural Language Processing (NLP) with RL, enabling researchers to address a combination of RL training and language-centric tasks effectively. Leveraging PyTorch's robust capabilities, OpenRL exemplifies modularity and a user-centric approach. It offers a universal interface that simplifies the user experience for beginners while maintaining the flexibility experts require for innovation and algorithm development. This equilibrium enhances the framework's practicality, adaptability, and scalability, establishing a new standard in RL research. To delve into OpenRL's features, we invite researchers and enthusiasts to explore our GitHub repository at https://github.com/OpenRL-Lab/openrl and access our comprehensive documentation at https://openrl-docs.readthedocs.io.

==> main_texts/2_related_work.tex <==
\section{Related Work}

Reinforcement learning (RL) libraries have experienced significant growth and development over the years. Many robust libraries such as Stable Baselines3~\citep{stable-baselines3}, Rllib~\citep{liang2018rllib} and rlpyt~\citep{stooke2019rlpyt} have set a strong foundation for RL research, each offering its unique advantages. Nevertheless, certain experiences with these libraries have highlighted areas in which we believe our new framework, OpenRL, could particularly shine.
Stable Baselines3 streamlines ease of use and introspective documentation but seems to sacrifice modularity. While it's tailored towards the single-agent landscape, it lacks something to address the complexity of multi-agent scenarios, self-play training, or the emerging NLP/RL hybrid fields, all of which OpenRL seamlessly integrates.
Though Rllib supports multi-agent training and exhibits favorable scalability, it comes with a more complex codebase and could be unnavigable for novices. Conversely, in OpenRL, our design philosophy affords the user a simpler, unambiguous experience while preserving ample potential for expert tinkering.
The modular-based rlpyt and other adherents of this design approach, like Tensorforce~\citep{tensorforce} and MushroomRL~\citep{d2021mushroomrl}, are powerful tools empowering users in the rapid amalgamation of assumptions from different papers. However, the trade-off is often a steep learning curve wherein novice users must comprehend the entire code structure before gaining the capability to modify it. In contrast, OpenRL provides a harmonious balance between new user experiences and expert access to customization.
Frameworks such as d3rlpy~\citep{seno2022d3rlpy} and TimeChamber~\citep{inspirai} provide tools for specific research strains—offline RL and self-play, respectively—but lack broad generalizations to other areas of RL. OpenRL takes on a more holistic approach, providing the community with an inclusive environment that supports various RL scenarios while specifically excelling in the realms of self-play and NLP/RL convergence.
Moreover, gaining insight into the behavior and performance of RL agents over time can be a daunting task without ample documentation—a feature many libraries often neglect. OpenRL prioritizes bilingual documentation, making it more accessible and user-friendly for a global audience.
The above comparison primarily serves to illustrate the areas where OpenRL holds unique advantages. However, it's worth noting that we applaud the achievements and contributions of all these frameworks to the RL community. An in-depth comparison of our framework with other RL libraries is captured in Appendix~\ref{ap:lib_compare}.
